Scalable Neural Network Decoders for Higher Dimensional Quantum Codes

Machine learning has the potential to become an important tool in quantum error correction as it allows the decoder to adapt to the error distribution of a quantum chip. An additional motivation for using neural networks is the fact that they can be evaluated by dedicated hardware which is very fast and consumes little power. Machine learning has been previously applied to decode the surface code. However, these approaches are not scalable as the training has to be redone for every system size which becomes increasingly difficult. In this work the existence of local decoders for higher dimensional codes leads us to use a low-depth convolutional neural network to locally assign a likelihood of error on each qubit. For noiseless syndrome measurements, numerical simulations show that the decoder has a threshold of around $7.1\%$ when applied to the 4D toric code. When the syndrome measurements are noisy, the decoder performs better for larger code sizes when the error probability is low. We also give theoretical and numerical analysis to show how a convolutional neural network is different from the 1-nearest neighbor algorithm, which is a baseline machine learning method.

==> analysis_cnn_old.tex <==
\label{appendix:analysis_larger_network}

In the paper, the convolutional neural networks we use only have one convolution layer with kernel size $3^4$ and others are $1^4$. Therefore each element in the output (before applying softmax) is determined by its surrounding $3^4$ region. This is mainly for the sake of fast training and evaluation.
%Indeed, based on current technology of manufacturing qubits or classical computation speed, it is not practical to build a neural networks of much more layers or equivalently for each qubit to look at a much larger region around it.
However, it is still interesting to ask what will happen if we have a deeper neural network, especially considering the recent success of deep neural networks in image classification and processing.
More concretely, we wish to know if we increase the number of convolution layers (and as a result increase the region each qubit can ``look around'' to decide its error probability), will the machine learning procedure described in our paper perform better?
In the previous section we give an example that a nearest neighbor algorithm performs worse on a larger region. And in theory a deeper neural network will have a better ability to remember all the training data, thus has the capacity to be a nearest neighbor algorithm.
Therefore, it is important to try to understand some difference between how neural nets and nearest neighbor algorithm generalize to unknown inputs.
While there are likely many, in this section we will point out one particular difference between convolutional neural networks(CNN) and the nearest neighbor algorithm, resulted from the initialization and training of the networks.

In \autoref{fig:1d_conv} we draw a $m=4$ layer 1-d CNN with $n=7$ input bits and 1 output bit. In the figure, $x_{ij}$ are the values of neurons (as well as inputs). 
%It is clear (?) that if the number of filters is allowed to be arbitrarily large, then the CNN can approximate any function. In particular, it can be a lookup table based on the training data. Thus, it is desirable to understand what a CNN will learn with gradient based training methods. To achieve this, 
We will first consider the following simplified situation:
\begin{enumerate}
	\item  There is no non-linear activation function applied in the middle of the network. $\tanh$ is applied after the final layer $x_{m1}$ (e.g. in the figure, applied on $x_{41}$ ). There is also no bias term in the network. So the last layer $x_{m1}$ is a linear combination of the input bits $\{x_{1i}\}$.
	For the ease of notation, the number of channels for each layer is set to $1$.
	\item  The neural network is not convolutional, but instead a normal NN with the same local connectivity as a CNN.
	\item  The input-output relation to be learned as $y=x_{11}=x_{1k}=\pm 1$, where $k=\lfloor n/2 \rfloor$, $y$ is the desired output, and the probabilities of being $1$ and $-1$ are both $0.5$. Other $x_{1i}$ are set to $0$. The cost function is $c=(y-\tanh x_{m1})^2$.
\end{enumerate}

It is obvious that the neural net can approximate the above input-output relation well by being a linear combination $x_{m1}=a_1 x_{11}+a_k x_{1k}$ with the weights satisfy $a_1+a_k \gg 1$.
We will argue that with gradient descent as training method, in general we will have $a_k> a_1$. In other words, the output of the network $y'=\tanh (x_{m1})$ will depends more heavily based on $x_{1k}$ compared to $x_{11}$. Operationally, this can be checked by setting $x_{11}\neq x_{1k}$.
As we never train the neural net with data that have $x_{11}\neq x_{1k}$, this can be considered as checking how the neural net generalize to unseen inputs.

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.5\linewidth]{simple_convnn}
	\caption{An illustration of the connectivity of a small 1D convolutional neural network. In this section, we set the number of channel to $1$. Thus, each $x_{ij}$ is a real number. The arrays represent dependence relation. For example, $x_{21}$ is a function of $x_{11},x_{12},x_{13}$, and in this section the function is simply a linear sum.}
	\label{fig:1d_conv}
\end{figure}
We will assume the weights $\{w_{i}\}$ are initialized with the same normal distributions which has mean $0$ and standard deviation $\sigma$. Since there is no non-linear activation function, we have
\begin{align}
x_{ij}=\sum_k a^{(ij)}_k x_{1k} 
\label{eq_linear_network_coefficients}
\end{align}
We will show that when the weights of the network are initialized, $\operatorname{Var}(a^{(ij)}_k)$ is proportional to the total number of paths from $x_{1k}$ to $x_{ij}$.
Let $p$ be any path from $x_{1k}$ to $x_{ij}$. We can think $p$ as the set of weights $w_i$ on the path. It is easy to show that
\begin{align}
	a^{(ij)}_k = \sum_p \prod_{w_i \in p} w_i \equiv \sum_p W_p
\end{align}
Note that for different path $p_1$, $p_2$, while $W_{p_1}$ is not independent of $W_{p_2}$, we have $\operatorname{Cov}(W_{p_1},W_{p_2})=0$.
Thus, 
\begin{align}
	\operatorname{Var}(a^{(ij)}_k )=  \sum_p \operatorname{Var}(W_p)
\end{align}	
More generally, we can formulate the above argument as the following observation:
\begin{observation}
	\label{obs_variance_prop_num_paths}
	Define $b_{(i_1j_1)}^{(i_2j_2)}=\sum_{p\in S} \prod_{w_k \in p} w_k$, where $S$ is the set of paths from $x_{i_1j_1}$ to $x_{i_2j_2}$.
	When the weights of the network are initialized, $\operatorname{Var}(b_{(i_1j_1)}^{(i_2j_2)})$ is proportional to the total number of paths in $S$.
\end{observation}
We want to use the variance to compare the magnitudes of $b_{(i_1j_1)}^{(i_2j_2)}$.
In order for this to work, one condition is that the distributions of $b_{(i_1j_1)}^{(i_2j_2)}$ should all have a ``regular shape'' (e.g. approximated by normal distribution).
In \autoref{fig_pathsum}, we plotted the distribution of $a_{\lfloor n/2 \rfloor}^{(m1)}$, which is defined in \autoref{eq_linear_network_coefficients}. Again $m$ is the layer of the network and $n$ is the size of input.
From this numerical experiment, it is likely that the probability distribution of $b_{(i_1j_1)}^{(i_2j_2)}$ will have a bell shape when $x_{i_1j_1}$ and $x_{i_2j_2}$ are reasonably far away.
Thus, the variances will provide us a very way to compare the magnitudes of $b_{(i_1j_1)}^{(i_2j_2)}$.
For example, this implies that in \autoref{fig:1d_conv}, $x_{32}$ likely has a larger dependence on the $x_{14}$ compared to $x_{31}$ on $x_{11}$.
Some other conditions will be needed if we want to make the above comparison rigorous.
However, we will skip further discussion on this topic and be contend with an incomplete analysis.
%Another condition we should check is that $b_{(i_1j_1)}^{(i_2j_2)}$ are not correlated in a malicious way


\begin{figure}
	\centering
	\includegraphics[width=0.75\linewidth]{paths_for_a_weight}
	\caption{All paths through the grey area contributes to the gradient of $w_i$, while only the path along the edge contributes to $w_j$ (assuming there is no path from $x_{1\lfloor n/2 \rfloor}$ to $w_j$).}
	\label{fig_paths_for_a_weight}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{dist_of_pathsum}
	\caption{The distribution of the outputs from 3 and 4 layer neural network when the weights are initialized. 600 numerical trials are done in order to plot each figure. The networks have the connectivity shown in \autoref{fig:1d_conv}. The only non-zero element we set in the input is the center element $x_{1 \lfloor n/2 \rfloor}=1$. Thus, what we are showing here is the distribution of $a_{\lfloor n/2 \rfloor}^{(m1)}$, where $a_{k}^{(ij)}$ is defined in \autoref{eq_linear_network_coefficients} and $x_{m1}$ is the output of the network.}
	\label{fig_pathsum}
\end{figure}

We can use this approach to compare the gradients of the cost function $c$ with respect to different $w_i$.
The gradient sum over the two possible inputs $x_{11}=\pm 1$ is
\begin{align}
\sum_{x_{11}=\pm 1}\frac{\partial c}{\partial w_i} &= \sum_{x_{11}=\pm 1}\frac{\partial c}{\partial f} \frac{df}{d x_{m1}} \frac{\partial x_{m1}}{\partial w_i}
\end{align}
It is easy to see that 
\begin{align}
	\frac{\partial c}{\partial f} \left. \frac{df}{d x_{m1}}\right\rvert_{x_{11}=1}=-\frac{\partial c}{\partial f} \left. \frac{df}{d x_{m1}}\right\rvert_{x_{11}=-1}
\end{align}
and
\begin{align}
\frac{\partial x_{m1}}{\partial w_i} = \sum_{p \in S_i} \prod_{w_j \in p, j\neq i} w_j x_{11}
\end{align}
where $S_i$ is the set of paths which go through $w_i$ and one of $x_{11}$ and $x_{1\lfloor n/2 \rfloor}$.
Substitute these in, we have
\begin{align}
\label{eq:grad_final}
\sum_{x_{11}=\pm 1}\frac{\partial c}{\partial w_i} =2 \frac{\partial c}{\partial f} \left. \frac{df}{d x_{m1}}\right\rvert_{x_{11}=1} \sum_{p \in S_i} \prod_{w_j \in p, j\neq i} w_j
\end{align}
Since the first two terms on the r.h.s are the same when we compute $\frac{\partial c}{\partial w_i}$ for different $w_i$ in the same network, to compare the gradients we only need to consider the last term.
By using Observation~\ref{obs_variance_prop_num_paths}, we know that just after the initialization (or when $w_i$ have not been too correlated), the gradient of the weight that involved in more paths connecting $x_{11}$ or $x_{1\lfloor n/2 \rfloor}$ to $x_{m1}$ has a larger variance, and obviously the mean of the gradients are $0$.
On a speculation level,  this means most weights connecting $x_{1\lfloor n/2 \rfloor}$ to $x_{m1}$ changes faster compared to those connects $x_{11}$ to $x_{m1}$ in the same layer. Intuitively, this trends will continue, since the gradient w.r.t to a weight will be larger if other weights on the path have larger absolute values.

Now let us discuss the simplification we made above.
If the network is convolutional, which means the weights will be shared in the same layer, then the above argument need to be modified as apparently the weights are changing at the same rates regardless of its position in one layer.
However, Observation~\ref{obs_variance_prop_num_paths} still holds, because we still have $\operatorname{Cov}(W_{p_1},W_{p_2})=0$ for any two different paths $p_1$ and $p_2$.
Assume in the Fig~\ref{fig_paths_for_a_weight}, $w_i$ and $w_j$ are shared weights and thus $w_i=w_j$.
Let us consider the possible scenario that the gradient with respect to $w_i$ and $w_j$ have different signs, but the norm of the gradient w.r.t $w_i$ is much larger.
Then the update of $w_i$ (and $w_j$) will be according to the gradient of $w_i$, which increase the likelihood of the final decision $x_{m1}$ to be based on $x_{1\lfloor n/2 \rfloor}$.

The effect of activation function in the middle of the network will depend on the choice of the particular function and the initial distribution of the weights.
For example, if we initialize all weights with a small enough variance, then initially all $x_{ij}$ are still in the linear regime of activation function such as sigmoid or $\tanh$.
For the popular \textsc{relu} activation function (i.e. $y=\max (x,0)$), since it is linear whenever the input is larger then $0$, we can expect observation~\ref{obs_variance_prop_num_paths} to still be true.

Lastly, we considered a very simple input probability distribution. In general, the inputs are likely to be noisy, and the input-output relation is more complicated than an identity function. To have an toy example of noisy inputs, later in the next subsection we are going to perform a numerical experiment where we replace the $0$ input bits to a random $\pm 1$ in the input distribution we considered above. Intuitively, we can still argue that for $x_{ij}$ in the middle of a layer will have a larger signal-to-noise ratio compared to the ones on the edge, as a larger part of the variance come actually from the signal. This might suggest that the weights in the middle will change faster.

\subsection{Numerical results}

We setup the network and the training data according to the description above, with the only change being that inputs are 2D with size $7\times 7$ and $9\times 9$. The number of channels for each hidden layer is $10$. We choose one of the corner input bits to be the same (or reverse) of the center bit. The weights of the network are initialized with normal distribution that has mean $0$ and standard variance $0.1$. We use the vanilla gradient descent with some exponential decay of the learning rate. The final output of the $\tanh$ is rounded to integer and compared to the desired output. The training stops when the average of cost function $c$ is smaller then $0.02$ for a batch of 100 training data (the threshold of $0.02$ is chosen so that when given the reversed input, the output of $\tanh$ will be rounded to $\pm 1$ instead of $0$). We then test the network on inputs where the chosen corner bit and the center bit have different signs.

We repeat the above procedure for 20 times on both $7\times 7$ and $9\times 9$ inputs. In all experiments, the network always output the center input bit when the center and corner input bits have different sign.

We also do a test where the scenario is more complicated (and to some degree more practical). As discussed previously, we can add noise by changing all the $0$ in the inputs to a random $\pm 1$. \textsc{relu} activation function (i.e. $y=\max (x,0)$ is added to the middle layers of the network. The size of the input is $9\times 9$, and accuracy is evaluated by comparing the signs of the final $\tanh$ to the desired outputs. 
Otherwise the setting is the same as in the previous experiment.
In Figure~\ref{fig:aligned_vs_reversed}, we plot the accuracy during the training process. We can see while the accuracy rises when given the aligned inputs (i.e. the particular corner bit and the center bit are equal), the network becomes more deterministically at outputting the center bit when given reversed inputs (i.e. the particular corner bit and the center bit have inversed sign).
The test are repeated several times where similar results are observed.

\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{aligned_vs_reversed}
	\caption{Accuracy of matching the center input bits during training. Inputs are noisy and there are non-linear activation functions for all layers.
	The blue solid line corresponds to the accuracy when given aligned inputs, while the orange dotted one corresponds to reversed inputs. Note that in order to differentiate the lines, the accuracy for reversed inputs is defined to be the percentage of output matching the corner bit. Thus towards the end of the training, the outputs almost always matching the center bits when given reversed input. The accuracy is evaluated on a batch of 50 inputs.}
	\label{fig:aligned_vs_reversed}
\end{figure}



\subsection{Behavior of a larger neural network trained as decoder}
\label{appendix:behavior_larger_network}
In this subsection, we will analyze the behavior of a larger trained neural network, and show that it coincide with the above intuition. The neural network has two convolution layer which kernel size is $3^4$.
Thus, each element in the output of the neural network can be influenced by a $5^4$ region, or around 2500 input bits.
Generally speaking, if we have large neural nets on this many input bits, overfitting is very likely to happen.
For our particular setup of convolutional neural networks, it is much harder to estimate how many training data are needed to avoid overfitting.
Nevertheless, it is still interesting to look at the following two facts:
\begin{itemize}
	\item The trained larger network has a similar performance when decoding noiseless syndromes compared to the network we use in the main text, but is not tested as extensively.
	\item The larger network exhibits the decay of sensitivity we mentioned in this section, although it is not clear whether it is caused by that mechanism. See Figure~\ref{fig:sensitivity_vs_dist} for the plot. In other words, each element in the output will change more if an input bit closer to it is being changed.
\end{itemize}
Note that the second fact partially explained the first one: if the input bits outside the $3^4$ region do not have much influence on the corresponding output bit, then the smaller neural network used in the paper can in principle approximate the same input-output relation.

\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{sensitivity_vs_dist}
	\caption{Sensitivity of the neural network output with respect to changing a single input bit. The neural network is trained to estimate the probability of an error happened on the center qubit. The X-axis is the distance between the single changed input bit and the center, induced by $L^1$-norm. For each distance, we pick a random input bit and evaluate the difference of output if we change that bit. This is repeated for 20 times and an average is computed.}
	\label{fig:sensitivity_vs_dist}
\end{figure}

==> introduction_alternative.tex <==
A full-featured quantum computer will rely on some sort of error correction as physical qubits are prone to the effects of environmental noise.
The currently preferred coding architecture is the surface code in which the qubits and their interactions form a planar square grid.
%A planar layout aids in the physical implementation as long-range connections are harder to engineer in many quantum computing architectures.

Quantum codes in which the physical qubits interact {\em as if} they were nearest neighbors in a higher-dimensional space can be implemented in lower dimensions once connectivity can be non-local.

Using neural network to decode 4D toric code has a few advantanges.
First, as we do not presume the error model but training neural networks with data,  it can automatically handle noise models to a certain degree. For example, it should be able to adapt to the noise model induced by its measurement circuit. % Niko: we don't consider any other error models so maybe this should not be the first point.
Second, neural network decoder might achieve a balance between fast local decoders with low thresholds~\cite{BDDTlocaldecoders} and slow global decoders with high thresholds~\cite{4drenormalization}. 
Finally, there is a possibility that we want to implement 4D toric code with an experiment setting inside a fridge.
As an example, for superconducting qubits, 4D toric code could still have uses as a top code in which the logical qubits encoded by a 2D surface code are used as elementary qubits.
In these scenarios, we can use fast and low-power neural network chips~\cite{Mnnhardware,Mintegratedcircuit,jouppi2017datacenter} to do decoding in a low temperature environment.

%A further disadvantage is the fact that an algorithm such as minimum-weight perfect matching has to run on a reasonably complex classical computer.
%This classical computer is either close to the qubits, e.g. inside a fridge, and produces thermal noise which increases the error rate, or further away which leads to an even larger increase in time-delay \cite{bluhmarchitecture}.
%Hence, it would be advantageous to have dedicated hardware which can be implemented using fast, low-power electrical components. 
%This would decrease the effective rate of errors which can occur during an error correction cycle.
%Neural networks are a good candidate for such dedicated hardware.
%Many specialized neural network chips have been manufactured~\cite{Mnnhardware,Mintegratedcircuit,jouppi2017datacenter}.

%For example, in \cite{Mintegratedcircuit} the authors report on an integrated circuit implementing a network of 1 million neurons on a $240\mu \mbox{m} \times 390 \mu \mbox{m}$ CMOS chip.
%The chip draws $20 \mbox{mW}/\mbox{cm}^2$ as compared to $50\mbox{W}/\mbox{cm}^2$-$100\mbox{W}/\mbox{cm}^2$ for a modern CPU or $30\mbox{W}/\mbox{cm}^2$ for an FPGA \cite{Thardwarecomparison}, thereby reducing potential thermal noise by orders of magnitude.

Using neural networks to decode the surface code has been suggested in earlier work \cite{torlai2016neural,varsamopoulos2017decoding,baireuther2017machine,krastanov2017deep}. 
However, an issue that has not been addressed so far is scalability: 
in previous approaches the neural network has to be re-trained for every system size, despite the fact that in general machine learning methods become problematic when the input space becomes too large.
\Xiaotong{Thus, it is interesting to ask whether a scalable decoder exists for 4D toric code, which can be naturally represented by a neural network.}
Our contribution is the following:

\begin{itemize}
	\item We propose a decoder for the 4D toric code (and as a byproduct, a decoder for the sheet-like logical operator of the 3D toric code), which contains a low-depth convolutional neural network trained to locally assign a likelihood of error on each qubit as a subroutine. Due to the translational invariance of the neural network, it is sufficient to train it on a fixed size lattice and can then be scaled up to arbitrarily large system sizes, which avoids possible complication from machine learning.
%    Our approach should also work for hyperbolic surface code~\cite{Hdecoding,breuckmann2017hyperbolic}.
	\item For noiseless syndrome measurements, we observe the decoder to have a threshold around $7.1\%$ with 4D toric code in numerical simulations. When the syndrome measurements are noisy, the decoder still performs better for larger lattice when error probability is low, see \autoref{fig:memory_time} for the plot. More numerical simulation needs to be done to determine the threshold. 
	\item We give a toy example which shows how a baseline machine learning model can fail at a task similar to decoding when the system size becomes large. This highlights the importance of choosing a translational invariant model as we do. In addition, we observed and analyzed one property of multi-layer convolutional neural networks, and show it fits nicely to the task of assigning likelihood of qubit errors for high dimensional toric code.
\end{itemize}

%The reason we consider higher dimensional surface codes is that they have a few attractive features for a machine learning decoder, e.g. they have local and single-shot decoders.
%To some degree, this paper can be viewed as a proof of principle that neural network decoder is a viable option even in the long term, when we possibly need codes with large distance.

%In fact, classical computers already use non-local connectivity:
%A famous example is the supercomputer ``Connection Machine 2'' build in 1987 by the company ``Thinking Machines.''
%Its internal connectivity is that of a 12-dimensional hypercube~\cite{connectionmachine}.

%Here we address the scalability problem by borrowing ideas from image recognition.
%Our networks are {\em convolutional neural networks} in which the number of parameters is constant with respect to the system size.
%Our network only needs to be trained once and can then be scaled up to arbitrarily large system sizes.
%As our neural network decoder has a local structure we apply it to a quantum code for which the decoding problem can be solved locally: the four-dimensional toric code.
%We perform a numerical analysis of the performance of the decoder assuming both perfect and faulty syndrome measurements.
%Furthermore, we theoretically and numerically analyze the behavior of the neural network used in our decoder, which suggests that increasing the number of layers would likely improve its ability of locally assigning likelihood of error.

% Summary
This paper is structured as follows.
In \autoref{sec:previous} we discuss previous work in which machine learning was applied to decode quantum codes.
 In  \autoref{sec:4DTC} we give a review of the 4D toric code and its properties. In \autoref{sec:ML}, we provide a general introduction to machine learning. 
In \autoref{sec:ML_for_decoding} we describe the application of convolutional neural networks as a subroutine in our decoding algorithm.
In \autoref{sec:Num} we discuss the results of Monte-Carlo simulations.
In \aref{appendix:training_neural_network}, we give a short introduction to the backpropagation algorithm which we use to train the neural network.
The rest of the appendix is devoted to a theoretical analysis of convolutional neural networks, indicating that they are suitable models for our decoding procedure.

==> machine_learning_basics.tex <==
\label{sec:neural_network_basics}

To make this article as self-contained as possible we give a brief introduction to machine learning with neural networks.
For more background we refer to \cite{Mmachinelearning,Nmachinelearning,Gmachinelearning}.


A {\em neural network} is a directed, multipartite graph consisting of {\em layers} $l = 0,\dotsc,L$.
The vertices in layer $l$ are connected to vertices in the following layer $l+1$.

\begin{figure}[h]
    \begin{center}
        \includestandalone[scale=0.8,mode=buildnew]{figures/neural_network_schematic}
    \end{center}
    \caption{A neural network consisting of $3$ layers. The network takes input $x \in \{0,1\}^{m}$ which is represented as the first layer of neurons. The values of neurons in the hidden layer and the output layer are given by the function $f_{w,b}:\real^q \rightarrow [0,1]$ evaluated on their input (indicated by $q$ incoming arrows). The parameters $w \in \real^{q}$ and $b\in \real$, called weights and bias, can be different for each neuron. The values of the neurons in the last layer are the output of the network $F^N(x) \in \real^{n}$.}
    \label{fig:nnschematic}
\end{figure}

The vertices of the network are called {\em neurons}.
The main idea behind the neural network is the following:
Each neuron  computes a primitive non-linear function $f_{w,b}:\real^q \real$, for which the input values are given by neurons of the previous layer connected to it.
%In Fig. \ref{fig:nnschematic} all layers are fully connected.
%Later we will discuss networks with less connectivity.
The subscripts $w \in \real^{q}$ and $b\in \real$ are parameters which can differ for each neuron.
Before we discuss the function $f_{w,b}$ in more detail let us first understand how the network performs a computation.
%The number of inputs $q$ of a neuron is given by the number of incoming edges.
The neurons in the first layer do not have any predecessors and their output is simply set to be the input of the network, which is a bit string $x \in \{0,1\}^{m}$.
The values of the neurons in the last layer are interpreted as the output of the network.
We see that the network describes a function $F : \{0,1\}^{m} \rightarrow [0,1]^{n}$.
The first layer $l=0$ is called the {\em input layer} and the last layer $l=L$ is called the {\em output layer}.
All other layers $l = 1,\dotsc,L-1$ are called {\em hidden layers} since they are considered to be internal to the network.

The parameters $w$ and $b$ are called {\em weights} and {\em biases}.
They define a linear map $w\cdot y + b$ where $y$ is the input of the neuron.
The function that each neuron computes has the form:
\begin{align}
    f_{w,b}:\real^q \rightarrow [0,1],\quad x \mapsto \sigma(w\cdot y + b)
\end{align}
where in this paper $\sigma$ is either $\tanh$ or the {\em sigmoid function}
\begin{align}
    \sigma(z) = \frac{1}{1+\exp(-z)}
\end{align}
which is plotted in Fig. \ref{fig:sigmoid}.
Both non-linear functions can be thought of as a smoothed step function.
The smoothness of $\sigma$ is important to the training of the neural networks as .

\begin{figure}[h]
    \begin{center}
        \begin{tikzpicture} 
        \begin{axis}[xmin=-5,xmax=5,no markers,samples=50,grid=both]
        \addplot {1/(1+exp(-x))} node[below left]{$\sigma(z)$};
        \addplot[domain=-5:0] {0} node[right]{$\Theta(z)$};
        \addplot[dashed]  coordinates {(0,0)(0,1)};
        \addplot[domain=0:5] {1};
        \end{axis}
        \end{tikzpicture}
    \end{center}
    \caption{The sigmoid function $\sigma$ is a smooth version of the Heaviside step function $\Theta$.}
\label{fig:sigmoid}
\end{figure}


Let us have a look at a small example which gives some intuition why neural networks are able to perform interesting computations:
Consider a single neuron which takes $q = 2$ inputs and has weights $w = (-12,-12)$ and bias $b = 17$.
The neuron computes the following values for each input:
\begin{align}
\begin{split}
    f(0,0) &= \sigma(17) \approx 1\\
    f(1,0) &= \sigma(5) \approx 1\\
    f(0,1) &= \sigma(5) \approx 1\\
    f(1,1) &= \sigma(-7) \approx 0.
\end{split}
\end{align}
We observe that these are approximately the input/output relations of the NAND gate.
The approximation can be made arbitrarily close by increasing the absolute values of the weights $w$ and the bias $b$.
Since any Boolean function $F : \{0,1\}^m \rightarrow \{0,1\}^n$ can be computed by a network of NAND gates, there consequently also exists a representation of $F$ as a neural network.
However, in practice it is more efficient to adapt the connectivity of the network to the problem at hand.


\subsection{Convolutional Layers in Neural Network}
\label{sec:CNN}
In this subsection we will explain what is a convolutional layer in a neural network. To begin with, the input to the layer need to reside on a $D$-dimensional lattice of size $L^D$.
On each lattice site, there is a $d$-dimensional vector $x_\mathbf{u} \in \real^d$, where the subscript $\mathbf{u} \in \mathbb{Z}_L^D$ (we use $\mathbb{Z}_L$ to denote integer in range $[0,L-1]$).
We define the kernel to be a vector $K_{\mathbf{u},i}$, where $\mathbf{u} \in \mathbb{Z}_n^D$ and $i \in \mathbb{Z}_d$. The convolution is then
\begin{align}
\label{eq:convolution}
y_\mathbf{v} = \sum_{\mathbf{u} \in \mathbb{Z}_n^D, i \in \mathbb{Z}_d} x_{v-u, i} K_{u, i},
\end{align}
where $x_{v-u,i}$ is the $i$th element of $x_{v-u}$, and each element of $\mathbf{v}$ has range $[n-1, L-1]$.
The index $v$ of the output $y$ can be shifted according to needs (e.g. to $\mathbb{Z}_{L-n+1}^D$).
In this paper, we solely work with input that has the periodic boundary condition.
Thus, we can indeed treat the indices $\mathbf{u}$ of input $x_\mathbf{u}$ as elements of the cyclic group $\mathbb{Z}_L^D$.
The convolution~\eqref{eq:convolution} can then be modified accordingly such that $\mathbf{v} \in \mathbb{Z}_L^D$.
If there are multiple kernels, we can apply Equation~\ref{eq:convolution} for each kernel individually, then stack the outputs together in the natural way.
Non-linear functions can be applied after convolution if needed.
In this paper, convolutional neural networks are neural networks with only convolutional layers.

The connectivity of a 1-D convolutional neural networks is illustrated in Figure~\ref{fig:1d_conv}.
It is easy to see that a convolutional layer~\eqref{eq:convolution} is simply a neural network layer with local connectivity and the weights are translational invariant.



==> qip_introduction.tex <==
%\Xiaotong{my thoughts on the two introduction: I think it basically boils down to question that, 10 years later, do you think people care more about using machine learning to do decoding, or use 4D toric code for quantum computation.}


As quantum error correction is a very demanding task for hardware, it is worth optimizing the procedure in the experiments. 
Apart from tuning control parameters that implement different gates, the decoding algorithm should also be tailored to the noise introduced by these gates and the error correcting circuits. 
The optimization of the decoding algorithm can be a lengthy task, and it can even be a hard one when subjected to certain constraints. For example, many fault-tolerant quantum computation architectures require real-time decoding, which means the decoder has to be extremely fast.
A rough calculation \cite{Tftreview} shows that assuming a quantum error correction cycle of $5\mbox{MHz}$ for an $L = 100$ surface code the classical decoder needs to process the measurement information at $100 \mbox{Gbit/s}$.

It is thus beneficial to find a way that automatizes the optimization of decoders. This can be done, for instance, by replacing subroutines of a decoder with certain machine learning models, and then these models are trained for the decoder to achieve the best performance. 
Ideally, not only the training process should be efficient in terms of computational complexity, but the human effort involved in selecting models and training should also be manageable. 
The family of neural networks is a good candidate for the machine learning models, as they are flexible, fast to evaluate and have good software packages. 
Moreover, it is possible to have specialized chips for neural network evaluation, which offers additional versatility to the experimental setups, e.g. bypass the need of connecting to full-featured classical computers.

However, if the subroutine which we want to optimize is reasonably complicated, then it is hard to guarantee the quality of the obtained solutions. 
Since in the long term, we will want to use codes with large size to reduce the error rate, we should consider the scalability of using machine learning to optimize decoding algorithms. 
A good starting point to achieve the scalability is to consider families of quantum codes with certain symmetries, for which we only need to optimize subroutines with fixed input size. 
Possible examples are topological codes and concatenated quantum codes.

Our contribution:

\begin{itemize}
	\item We propose an architecture of decoder for 3D and 4D toric code, which contains a low-depth convolutional neural network trained to locally assign a likelihood of error on each qubit as a subroutine. Due to the translational invariance of the neural network, it is sufficient to train it on a fixed size lattice, which avoids possible complication from machine learning.
	\item For noiseless syndrome measurements, we observe the decoder to have a threshold around $7.1\%$ with 4D toric code in numerical simulations. When the syndrome measurements are noisy, The decoder still performs better for larger lattice when error probability is low. 
	\item We give a toy example which shows how a common machine learning model can fail at a task similar to decoding when system size grows large. This highlights the importance of choosing a translational invariant model as we do. In addition, we observed and analyzed one property of multi-layer convolutional neural networks, and show it fits nicely to the task of assigning likelihood of qubit errors for high dimensional toric code.
\end{itemize}
